Combining Priors with Experience: Confidence Calibration Based on Binomial Process Modeling

Confidence calibration of classification models is a technique to estimate the true posterior probability of the predicted class, which is critical for ensuring reliable decision-making in practical applications. Existing confidence calibration methods mostly use statistical techniques to estimate the calibration curve from data or fit a user-defined calibration function, but often overlook fully mining and utilizing the prior distribution behind the calibration curve. However, a well-informed prior distribution can provide valuable insights beyond the empirical data under the limited data or low-density regions of confidence scores. To fill this gap, this paper proposes a new method that integrates the prior distribution behind the calibration curve with empirical data to estimate a continuous calibration curve, which is realized by modeling the sampling process of calibration data as a binomial process and maximizing the likelihood function of the binomial process. We prove that the calibration curve estimating method is Lipschitz continuous with respect to data distribution and requires a sample size of $3/B$ of that required for histogram binning, where $B$ represents the number of bins. Also, a new calibration metric ($TCE_{bpm}$), which leverages the estimated calibration curve to estimate the true calibration error (TCE), is designed. $TCE_{bpm}$ is proven to be a consistent calibration measure. Furthermore, realistic calibration datasets can be generated by the binomial process modeling from a preset true calibration curve and confidence score distribution, which can serve as a benchmark to measure and compare the discrepancy between existing calibration metrics and the true calibration error. The effectiveness of our calibration method and metric are verified in real-world and simulated data.

==> img/Makefile <==

.SECONDEXPANSION:

.PRECIOUS: %.png %.pdf

.PHONY:	clean all

# OSX needs "." and does not accept POSIX "-o" flag

all:    $(shell find . -name "*.svg" | sed -e s/svg/xbb/g ) \
	$(shell find . -name "*.png" | sed -e s/png/xbb/g ) \
	$(shell find . -name "*.jpg" | sed -e s/jpg/xbb/g )

%.xbb : %.jpg Makefile
	ebb -x $<

%.xbb : %.png Makefile
	ebb -x $<

%.xbb : %.pdf
	ebb -x $<

# due to a bug in X11 on OSX, inkscape always requires absolute pathname
%.pdf : %.svg
	inkscape -f $(CURDIR)/$< -A $(CURDIR)/$*.pdf -d 150 || inkscape -o $(CURDIR)/$*.pdf -d 150 $(CURDIR)/$<
# %.png : %.svg
# 	inkscape -f $< -e $*.png -d 150
#	convert $< $*.png
#	if you want to use imagemagick, comment out 'inkscape...' and use 'convert...'

clean:
	-find . -name "*.xbb" -delete
	-rm *.png *.pdf

